Benchmarking Quantum Machine Learning for Power-System Attack Detection: Evaluation Choices Can Decide the Outcome

Quantum machine learning is proposed to detect grid cyberattacks, but no study we could read tests quantum and classical detectors under white-box, transfer, and black-box attacks and random label flips in one protocol. We compare two quantum and six classical detectors on public grid-attack data under equal tuning budgets. Our main finding: evaluation choices can decide the outcome. On these data, seven choices each changed a reported result with model families fixed. Row-level splits inflate our best score by 0.31 macro-averaged F1 over held-out files, where matched-dimensionality classical and quantum models barely clear chance. Under its own white-box attack the quantum kernel's score falls from 0.56 to 0.01 (chance 0.50), while a transferred attack in the same run leaves 0.52. Trees admit no gradient-based white-box attack, so their attacked scores are upper bounds. These attack results use eight-dimension detectors under row-level splits. On gas-pipeline and simulated-grid data, neither quantum detector is more accurate or consistently more robust; three of the seven choices reproduce fully on gas data with one pressure feature log-scaled (two within noise), and none of the four checked on the grids does. Benchmarks should hold out whole files and give every model its own attack where possible. We release code and checklist.

==> sections/abstract_tsg.tex <==
\begin{abstract}
Quantum machine learning is proposed to detect grid cyberattacks, but no study we could read
tests quantum and classical detectors under white-box, transfer, and black-box attacks and
random label flips in one protocol. We compare two quantum and six classical detectors on
public grid-attack data under equal tuning budgets. Our main finding: evaluation choices can
decide the outcome. On these data, seven choices each changed a reported result with model families fixed.
Row-level splits inflate our best score by 0.31 macro-averaged F1 over held-out files, where
matched-dimensionality classical and quantum models barely clear chance. Under its own white-box
attack the quantum kernel's score falls from 0.56 to 0.01 (chance 0.50), while a transferred
attack in the same run leaves 0.52. Trees admit no gradient-based white-box attack, so their attacked scores are upper
bounds. These attack results use eight-dimension detectors under row-level splits. On
gas-pipeline and simulated-grid data, neither quantum detector is more accurate or consistently
more robust; three of the seven choices reproduce fully on gas data (two within noise), and none
of the four checked on the grids does. Benchmarks should hold out whole files and give every model its
own attack where possible. We release code and checklist.
\end{abstract}

